Iterative Volume-of-Fluid interface positioning in general polyhedrons with Consecutive Cubic Spline interpolation

A straightforward and computationally efficient Consecutive Cubic Spline (CCS) iterative algorithm is proposed for positioning the planar interface of the unstructured geometrical Volume-of-Fluid method in arbitrarily-shaped cells. The CCS algorithm is a two-point root-finding algorithm specifically designed for the VOF interface positioning problem, where the volume fraction function has diminishing derivatives at the ends of the search interval. As a two-point iterative algorithm, CCS re-uses function values and derivatives from previous iterations and does not rely on interval bracketing. The CCS algorithm only requires only two iterations on average to position the interface with a tolerance of $10^{-12}$, even with numerically very challenging volume fraction values, e.g. near $10^{-9}$ or $1-10^{-9}$. The proposed CCS algorithm is very straightforward to implement because its input is already calculated by every geometrical VOF method. It builds upon and significantly improves the predictive Newton method and is independent of the cell's geometrical model and related intersection algorithm. Geometrical parametrizations of truncated volumes used by other contemporary methods are completely avoided. The computational efficiency is comparable in terms of the number of iterations to the fastest methods reported so far. References are provided in the results section to the open-source implementation of the CCS algorithm and the performance measurement data.

==> sections/geometrical_algorithms.tex <==
\section{Geometrical algorithms}
\label{sec:geom}

The \emph{multiset} geometrical model is used to handle general polyhedrons that can be non-convex and have non-planar faces. The multiset model represents a geometrical object as a multiset of its sub-elements: a polygon is a set of line segments, a polyhedron is a set of polygons, a triangulation is a set of triangles or tetrahedrons. This greatly simplifies the topological operations, because the elements store their own geometrical data that can be directly modified. Storing own data in sub-sets repeats information, which gives the multiset model its name. For example, a triangle represented as a multiset of points $p_i$ could look like $T = \{(p_0,p_1),(p_1,p_2),(p_2,p_3)\}$. The the last edge of the triangle $(p_3,p_0)$ is not stored, it is simply used by an algorithm, if the set $T$ is considered as a triangle, and not used by an algorithm if $T$ is considered as an open chain of line segments. 

Repeating information may incur additional costs because more memory is used to store and fetch the data. This depends strongly on the algorithms that are applied on the model. However, the \texttt{geophase} library provided alongside this manuscript does not rely on a single geometrical model. It abstracts the models and can be easily extended to support other models such as \emph{indexed face sets} or \emph{graph-based models} \cite[chapter 26]{Ghali2008}. Moreover, a significant loss in computational efficiency caused by the multiset geometrical model has not been measured for the adveciton of the interface reported in \citep[tables 3,5 and 6]{Maric2018}. The computation times reported for the UFVFC-Swartz VOF method are comparable or shorter than those reported for contemporary structured VOF methods. The new iterative positioning algorithm described in \cref{sec:positioning} increases further the computational efficiency of the interface reconstruction. The main motivation for the current support of multiset models is the simplicity of the implementation of their respective geometrical algorithms. Up to the very recent publication by \citet{Lopez2019}, unstructured un-split VOF methods were developed for convex polyhedrons \citep{Maric2013,Jofre2014,Jofre2015,Maric2018} and non-convex polyhedrons were triangulated \citep{Chenadec2013,Ivey2017,Chen2017,Maric2018,Chen2019}. \citet{Lopez2019} achieve a fast implementation of intersection and volume calculation using the indexed face set boundary representation. 

\begin{table}[htb]
\centering
\caption{Elementary geometric algorithms}
\label{tab:elemgeo}
\begin{tabular}{lll}
\midrule
    distance$^p$       & equal$^p$            & extreme\_point$^g$ \\ 
    area$^g$           & signed\_distance$^g$ & orient$^p$          \\
    do\_intersect$^p$ & is\_inside$^p$        & triangulate$^g$    \\  
    centroid$^g$       & intersect$^g$        & volume$^g$         \\
\midrule
\end{tabular}
\end{table}

Elementary geometrical algorithms are listed in \cref{tab:elemgeo} and are applied on different geometrical models. They are categorized into \emph{predicates} (denoted with "$^p$") and \emph{generative} algorithms (denoted with "$^g$"). Geometrical predicates are functions with a Boolean return type: they are evaluated either as false, or true (\citep[chap. 2]{Ghali2008},\citep{Shewchuk2013},\citep[sec. 3.2]{Shewchuk2016}). Generative algorithms use (floating point) numbers as input, and generate (floating point) numbers as output. It is important to distinguish the two groups, because the generative algoirhtms used by the VOF depend on trustworthy geometrical predicates, that can robustly and quickly handle perturbations in data resulting from repeated calculations with floating point numbers. Handling numerical robustness with floating point operations is proposed in \cref{subsec:robustness}.

Elementary geometrical algorithms from \cref{tab:elemgeo} are combined to build to VOF-specific algorithms, such as: position\_interface$^g$, edge\_triangulate$^g$, flux\_triangulate$^g$, flux\_stencil$^g$, reconstruct\_interface$^g$, phase\_flux\_contribution$^g$, etc. The main elementary algorithm is the intersection between a polyhedron and a halfspace and the respective computation the volume of the intersection and the area of the \emph{cap polygon}: polygon of the intersection that lies on the halfspace. Triangulation of the polyhedron is used to handle possible non-convexity and non-planarity. For the intersection of halfspaces and star-shaped polyhedrons\footnote{A star-shaped polyhedron is a polyhedron that can be decomposed into tetrahedrons using an additional point.}, a centroid-based volume triangulation is used, outlined in \cref{alg:tri:centroid}. The line \cref{alg:tri:centroid:last} is an example of the implicit handling of the last edge to close a multiset polygon in \cref{alg:tri:centroid}. Not storing the last edge and unrolling the loop for the last iteration instead of checking for it only increases the implementation efficiency. The volume triangulation $Tr_c$ computed by \cref{alg:tri:centroid} is re-used whenever the interface is positioned in the polyhedron $V_c$. Note that the flux volumes computed by the unstructured un-split VOF method are not necessarily star-shaped and therefore require an alternative triangulation, such as the one proposed in \citep{Maric2018}.

\begin{algorithm}[htb]
    \centering
    \caption{Centroid-based volume triangulation}
    \label{alg:tri:centroid}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Polyhedron $V_c$ 
            \State \textbf{Returns:} Volume triangulation of $V_c$: a set of tetrahedrons $Tr_c = \{T_i\}$ 
            \State $Tr_c = \emptyset$
            \State Compute polyhedron centroid $\x_c = \frac{1}{|P_{c}|} \sum_{p=1}^{|P_{c}|} \x_p$ \Comment $P_c = $ set of polyhedron points.
            \For{$f = 1, f  < |F_c| - 1, f = f + 1$} \Comment $F_c = $ set of polyhedron faces.
                \State Compute polygon centroid $\x_f = \frac{1}{|P_{f}|} \sum_{p=1}^{|P_f|} \x_p $ \Comment $P_f = $ set of polygon points.
                \For{$g = 1, g  < |P_f| - 1, g = g + 1$} 
                    \State $Tr_c = Tr_c \ \cup$ \texttt{build\_tetrahedron}$(x_c, x_f, x_g, x_{g+1})$
                \EndFor
                \State $Tr_c = Tr_c \ \cup$ \texttt{build\_tetrahedron}$(x_c, x_f, x_{|P_f| -1}, x_{0})$ \label{alg:tri:centroid:last}
            \EndFor
            \State \Return $Tr_c$
      \end{algorithmic}
    }
\end{algorithm}

\begin{algorithm}[htb]
    \centering
    \caption{Triangulation / halfspace intersection}
    \label{alg:intersect:triangulation:hspace}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Volume triangulation $Tr_c = \{T\}$, volumes of the tetrahedrons $\{V_T\}$, halfspace $H_c$
            \State \textbf{Returns:} Intersection volume $|V_{c,H_c}|$, coplanar intersection area $|A_{c,H_c}|$
            \For{$i = 0, n  < |Tr_c|, i = i + 1$} \Comment For all tetrahedrons in the triangulation.
              \If {\texttt{do\_intersect\_error}$(T_i, H_c)$} \Comment If tetrahedron interesects halfspace. 
                  \State $T_{i, H_c} = $\texttt{intersect\_error}$(T_i, H_c)$
                  \If {$T_{i, H_c} \ne \emptyset$} \Comment Degenerate empty set cases not covered by error predicates.
                    \State $|V_{c,H_c}| = |V_{c,H_c}| + $ \texttt{volume\_by\_surf\_tri}$(T_{i, H_c})$
                    \State $A_{i,H_c} = $ last polygon in the $T_{i, H_c}$ multiset polyhedron. \Comment $A_{i,H_c}$ always convex. 
                    \State $|A_{c,H_c}| = |A_{c,H_c}| + $\texttt{area\_oriented}$(A_{i, H_c})$ 
                  \Else{} \Comment Tetrahedron inside halfspace.
                    \State $|V_{c,H_c}| = |V_{c,H_c}| + V_{T,i}, \quad V_{T,i} \in \{V_T\}$ \Comment Add a precomputed volume.
                  \EndIf
              \EndIf
            \EndFor
      \end{algorithmic}
    }
\end{algorithm}

The triangulation / halfspace intersection algorithm is shown in \cref{alg:intersect:triangulation:hspace}. \Cref{alg:intersect:triangulation:hspace} is a generative algorithm that reduces the computational costs by precomputing the volumes of the tetrahedra in the triangulation and using intersection test $\texttt{do\_intersect\_error}$, based on forward floating point error estimation, to check for intersection. This way, intersections are performed only for tetrahedra that are intersected with the halfspace, and the total volume of the intersection is increased by the precomputed tetrahedron volume for those tetrahedrons that are inside the halfspace. A polyhedron is denoted as $V_c$ and its respective halfspace $H_c$ is defined at a point $\p_c$ with the unit normal orientation vector $\n_c$ as  
%
\begin{equation}
    H_{c} := H_{c}(\p_{c}(t), \n_{c}(t)) = 
    \begin{cases} 
        1 \text{ if } (\x - \p_{c}(t)) \cdot \n_{c}(t) >= 0, \\
        0 \text{ otherwise.}
    \end{cases}
    \label{eq:hspace}
\end{equation}
%
and negative halfspace is $-H_c = H_c(\p_c, -\n_c)$. The intersection between the halfspace $H_c$ and the polyhedron $V_c$ is denoted as $V_{c,H_c} = V_c \cap H_c$. The co-planar intersection $A_{c, H_c} \subset V_c \cap H_c$ is the set of points that belongs to $V_c \cap H_c$ but lies on the halfspace $H_c$, namely  
%
\begin{align}
    A_{c, H_c} & = \{\x, \x \in V_c \text{ and } (\x - \p_{c}(t)) \cdot \n_{c}(t) = 0 \}, \\
               & = V_{c,H_c} \cap -H_c 
    \label{eq:caparea}
\end{align}
%
Note that $A_{c,H_c} \subset V_{c,H_c}$, so it is not necessary to compute it additionally. Both $V_c \cap H_c$ and $A_{c, H_c}$ can be composed of disjoint sets when non-convex polyhedrons are intersected (see \cref{fig:endofill} in \cref{sec:positioning}). Before describing the more complex intersection and intersection test algorithms, algorithms \texttt{vol\_surf\_tri} and \texttt{area\_oriented} are described. The \texttt{vol\_surf\_tri} algorithm computes a polyhedron volume with 
%
\begin{align}
    |V_c| & = \dfrac{1}{3} \int_{V_c} \nabla \cdot \x \, dx = \dfrac{1}{3} \int_{\partial V_c} \x \cdot \n \, do, \\
          & = \dfrac{1}{3} \left[ \sum_{f=1}^{|F_c|} \left( \int_{A_f} \x_f \, do + \int_{A_f} (\x  - \x_f) \, do, \right) \right] 
    \label{eq:areacentroid}
\end{align}
%
where $F_c$ is the set of boundary polygons $A_f$ (\emph{faces}) of the polyhedron $V_c$. If the centroid of $A_f$ is chosen as $\x_f$, the centroid definition $\int_{A_f} (\x  - \x_f) \, do = 0$ leads to 
%
\begin{equation}
    |V_c| = \dfrac{1}{3} \sum_{f=1}^{|F|} \x_f \cdot \Sf,  
    \label{eq:volume}
\end{equation}
%
where $\Sf = |A_f| \n_f, \|\n_f\|_2 = 1,$ is the surface area normal vector of the polyhedron face $f$. \Cref{eq:volume} (or another \emph{linear} volume calculation) cannot be used if the faces (sides) of the bounded volume are \emph{non-linear} (non-planar). The planarity of the faces is obtained by the multiset polyhedron representation because a triangulation is used to linearize the polyhedron faces. Using other representations, such as the indexed face-set, or graph-based boundary representation do not solve the isssue of a linear volume computation and intersection for polyhedra with non-planar (non-linear) faces. For non-planar faces, triangulation or other linear approximation of faces is required. Linearization is widely used to simplify the polyhedron geometry in the VOF context. \citet{Liovic2006} have linearized the non-planar faces of the flux polyhedrons to simplify geometrical operations in $3D$. \citet{Zhang2014} have linearized their polygons in order to increase the convergence order for the $2D$ volume fraction advection by increasing the sub-grid resolution of the interface and the temporal integration of the flux polygons. \citet{Jofre2014} have done it as well for flux polyhedra, \citet{Comminal2015} for the polygonal approximation of the cell pre-images as well in $2D$. 

The intersection of the tetrahedron with the halfspace, $T_{i, H_c} = T_i \cap H_c$ in \cref{alg:intersect:triangulation:hspace} is convex. Therefore, the cap polygon of $T_{i,H_c}$ is convex. That is why the contribution to the set $A_{c,H_c}$ may be computed with the straightforward \texttt{area\_oriented} \cref{alg:area:oriented}. 
%
\begin{algorithm}[htb]
    \centering
    \caption{Oriented area}
    \label{alg:area:oriented}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Polygon $A$ 
            \State \textbf{Returns:} Polygon area $|A|$ 
            \State $|A| = 0 $
            \For{$i = 1, i  < |P_i| - 1, i = i + 1$} 
                \State $|A| = |A| + 0.5 \|(x_{i} - x_0) \times (x_{i+1} - x_0)\|_2$
            \EndFor
            \State \Return $|A|$
      \end{algorithmic}
    }
\end{algorithm}
%

\subsection{Intersection and robustness}
\label{subsec:robustness}

Intersection and intersection test algorithms are very closely related to the topic of numerical robustness. Floating point predicates often return false results, because a small perturbation in values may result in a different result of a logical comparison. When a predicate fails, a false decision is made by the algorithms such as the intersection \cref{alg:intersect:triangulation:hspace} whether an entire geometrical model is intersected by the halfspace or not. This deserves a pause in consideration. Based on a very small perturbation, compared to the dimension of a geometrical model, a logical decision is made wether to keep or discard the whole geometrical model. Numerical robustness of geometrical computation is a broad topic. Overview information on this topic can be found in \citep{Fortune1996,Hoffmann2001,Kettner2008}, \citep[chap. 7]{Ghali2008}, \citep{Shewchuk2013}, \cite[chap. 45]{Toth2017} for computational geometry, and for computer graphics in \citep[chap. 11 and 12]{Ericson2004}.  

Numerical robustness can be improved by bounding errors with interval arithmetic (\cite{Duff1992,Snyder1992,Hu1995, Hu1996a}), adaptive precision predicates (\cite{Shewchuk1997,Levy2016}), or tolerance-based approaches (\cite{Segal1990,Edelsbrunner1990,Jackson1995,Cazals1997,Qi2006,Zhang2007}). Alternatively, exact calculations are used that rely on exact predicates (\cite{Fabri1996, Li2005, Hachenberger2007}). The bounds of the errors set by interval arithmetic tend to be too pessimistic, and the interval arithmetic incurs additional operations to bound the error. Adaptive precision predicates deliver a compromise between the expensive exact floating point arithmetic and unreliable use of tolerances, by resolving floating point computations up to bounded error margin. Tolerance-based approaches are fast, but usually reliable only for the tests they are tuned to. Exact predicates extend the floating point number system in order to support arbitrary precision. Exact predicates are of course most reliable, but are computationally the most expensive option.

The high accuracy of the geometrical VOF increases computational costs. For example, using only $10\%$ of a total of $1e05$ polyhedrons per CPU to represent the fluid interface, requires $10000$ polyhedrons $\times 4$ halfspace / polyhedron intersections just for interface positioning (see \cref{sec:positioning}), in the worst case. To evolve the fluid interface, advection on a hexahedral mesh requires $10000\times6$ (flux faces) $\times 18$ (flux stencil cells) $\times 6$ (faces per stencil cell) polyhedron / halfspace intersections, resulting (together with positioning) in $6520000$ halfspace-polyhedron intersections \emph{per single time step of simulation time}, in the worst case. Therefore, the approach that increases the trustworthiness of the VOF method must do so without significantly increasing the computational costs and making the $3D$ implementation intractable. This estimate already rules out the use of exact predicates and topology-preserving algorithms that are based on them. The robustness of the geometrical VOF method is further reduced by the composition of intersections between polyhedrons and halfspaces (intersection denoted with $I$), for computing phase flux volume contribution $V_{f,\alpha}$ (see \citep[eq. 32]{Maric2018}) as
%
\begin{equation}
    V_{f,\alpha} = V_f^r \mapsfrom I^{r-1}(V_f^{r-1}, H_{r-1}) \mapsfrom \dots \mapsfrom V_f^1 \mapsfrom I^0 (V_{f}^{0}, H_0).
    \label{eq:intercompos}
\end{equation}
%
\Cref{eq:intercompos} introduces error propagation from $r$ intersections, on top of the floating point robustness issue of geometric predicates. Adaptive predicates are fast but do not resolve the issue of disregarding those geometries that are produced by generative algorithms and are very close to each other. For example, if the use of adaptive predicates results in a line segment whose intersection will contain points below the adaptive precision of the predicate, repeated intersection of such result may not work. The errors calculated in different interval arithmetic approaches are difficult to bound and the tolerance-based approaches are forever associated with the tests used to callibrate them. The approach proposed here increases numerical robustness using forward rounding error propagation to set the bounds on the \texttt{do\_intersect\_epsilon} predicate from \cref{alg:intersect:triangulation:hspace}. This, together with \emph{geometry welding} \citep[chap. 12]{Ericson2004} from computer graphics is used to ensure topological consistency of the output in \cref{eq:intercompos} when \cref{alg:intersect:triangulation:hspace} is used as the intersection algorithm to accurately compute $V_{f,\alpha}$ from \citep{Maric2018}. 

The forward error analysis used in \texttt{do\_intersect\_epsilon} relies bounding the error of floating point arithmetic operations involved int computing the distance between a halfspace and a point. This is done based on the unit roundoff error of the IEEE754 double precision binary floating point format \cite[page 32]{Overton2001}, \cite[page 24]{Muller2010}, in the following way. Each floating point operation is expressed using the relative rounding error as 
%
\begin{equation}
    \begin{aligned}
        x \oplus  y  & = (x + y) (1 + \epsilon), \\
        x \ominus y  & = (x - y) (1 + \epsilon), \\ 
        x \otimes y  & = (x \cdot y) (1 + \epsilon), \\
        x \oslash y  & = (x \div y) (1 + \epsilon), 
    \end{aligned}
    \label{eq:round}
\end{equation}
%
such that $|\epsilon|<0.5\cdot2^{-p + 1}$, when rounding to nearest mode is used with $p=53$, the precision of the double precision binary floating point format. Operations $\oplus,\ominus,\otimes,\oslash$ are floating point operations. Forward error analysis inserts the floating point arithmetic operations into the expression for the signed distance between a halfspace $H$ and a point $\p$
%
\begin{equation}
    \delta_s := \delta_s(\r, H(\p,\n)) = (\r - \p) \cdot \n, \quad \|\n\|_2 = 1,
    \label{eq:signdistex}
\end{equation}
%
leading to the floating point signed distance,
\begin{equation}
    \delta_f := \delta_f(\r, H(\p,\n)) = (\r \ominus \p) \odot \n, \quad \|\n\|_2 = 1.
    \label{eq:signdistfl}
\end{equation}
%
The error between the exact and the floating point signed distance is expressed as
\begin{equation}
    \epsilon_{\delta} = \delta_s - \delta_f 
    \label{eq:sigdisterr}
\end{equation}
%
Algebraic expressions that appear in \cref{eq:sigdisterr} involve the individual components of $\r,\p,\n$ and $\epsilon_i$, a rounding error for each floating point operation. Introducing different $\epsilon_i$ in \cref{eq:round} is not necessary, it is done however to simplify the symbolic calculation. Namely, because the expressions are lengthy, they have been computed using the \texttt{sympy}\cite{sympy} Python library for symbolic mathematics.\footnote{The Sympy Jupyter notebook for the forward error analysis is available at \url{http://dx.doi.org/10.25534/tudatalib-71}.}  From \cref{eq:sigdisterr} a bound on the error can be estimated as follows. Applying the triangle inequality on \cref{eq:sigdisterr} leads to 
\begin{equation}
    |\epsilon_{\delta}| = |\delta_s - \delta_f| \le \sum_{i = 1}^6 |\epsilon_i| |E_i|,
    \label{eq:sigdistabs}
\end{equation}
%
for the $6$ floating point operations used in \cref{eq:signdistex}: $3$ for the difference $\ominus$ and $3$ in the scalar product $\odot$. The $E_i$ term is an algebraic expression resulting from the factorization with $\epsilon_i$. The final expression for the error is obtain by substituting 
%
\begin{displaymath}
    |e_i| \le 0.5 \epsilon, \epsilon = 2^{-p + 1}
\end{displaymath}
%
into \cref{eq:sigdistabs}, resulting in
%
\begin{equation}
    \begin{aligned}
        |\epsilon_\delta| \le 0.5 \epsilon  ( &  
        \left|{n_{0} p_{0} - n_{0} r_{0}}\right| + 
        \left|{n_{1} p_{1} - n_{1} r_{1}}\right| +  
        \left|{n_{2} p_{2} - n_{2} r_{2}}\right| + \\
        & \left|{n_{0} p_{0} - n_{0} r_{0} + n_{1} p_{1} - n_{1} r_{1}}\right| + \\
        & \left|{n_{0} p_{0} - n_{0} r_{0} + n_{1} p_{1} - n_{1} r_{1} + n_{2} p_{2} - n_{2} r_{2}}\right| + \\
        & \left|{n_{0} p_{0} + n_{0} r_{0} - n_{1} p_{1} + n_{1} r_{1} - n_{2} p_{2} + n_{2} r_{2}}\right| )
    \end{aligned}
    \label{eq:signdisterrabs}
\end{equation}
%
Which gives a forward error estimate for the absolute signed distance used by the \texttt{do\_intersect\_error} algorithm used in \cref{alg:intersect:triangulation:hspace} and outlined in \cref{alg:dointersecterror}.

\begin{algorithm}[htb]
    \centering
    \caption{Is polyhedron intersected with a halfspace}
    \label{alg:dointersecterror}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Polyhedron $V_c$, Halfspace $H_c$
            \State \textbf{Returns:} Boolean \textbf{True} or \textbf{False}
            \For{polygon $P$ in poyhedron $V_c$} 
                \State $S(\r_0, H_c) = $ \texttt{is\_inside\_error}($\r_0$, $H_c$). \Comment $\r_0=$ first point in polygon $P$.
                \For{point $\r$ in polygon $P$} 
                    \State $S(\r, H_c) = $ \texttt{is\_inside\_error}($\r$, $H_c$).
                    \If{$((S(\r, H_c) != \texttt{COINCIDENT}) \text{ and } (S(\r, H_c) != S(\r_0, H_c)))$}
                        \State \Return \textbf{True}
                    \EndIf
                \EndFor
            \EndFor
            \State \Return{\textbf{False}}
      \end{algorithmic}
    }
\end{algorithm}

The \texttt{is\_inside\_error} algorithm uses the \texttt{signed\_distance\_error} that returns the floating point signed distance given by \cref{eq:signdistex} together with the absolute signed distance error estimate given by \cref{eq:signdisterrabs}. The \texttt{is\_inside\_error} algorithm then uses those two values to define the status of a point $\r$ with respect to the halfspace $H(\p,\n)$ as 
%
\begin{equation}
    S(\r,H(\p,\n)) =
        \begin{cases}
            \texttt{INSIDE}, \quad  \delta_s(\r,H(\p,\n)) > 0 \text{ and } \delta_s(\r,H(\p,\n))  - |\epsilon_\delta| > 0  \\
            \texttt{OUTSIDE}, \quad \delta_s(\r,H(\p,\n))  < 0 \text{ and } \delta_s(\r,H(\p,\n))  + |\epsilon_\delta| < 0 \\
            \texttt{COINCIDENT}, \quad \text{otherwise}.
        \end{cases}
    \label{eq:pointstatus}
\end{equation}
%
Instead of relying on a globally prescribed tolerance, tuned to a set of test cases \cref{eq:pointstatus} determines wether a point $\r$ is \texttt{INSIDE,OUTSIDE} or \texttt{COINCIDENT} with respect to a halfspace $H(\p,\n)$ based on the estimate of the absolute error in the signed distance calculation given by \cref{eq:signdisterrabs}. Points that are detected as \texttt{COINCIDENT} during the intersection process are handled to prevent duplication of data. In order to save computational resources, intersections are avoided for models that are within the halfspace and have elements (faces or points) that are lie on the halfspace, because their intersection with the halfspace has zero volume. That is why \cref{alg:dointersecterror} only returns \textbf{True} if a point pair exists such that one point is outside and the other is inside the halfspace as defined by \cref{eq:pointstatus}. 

Following \cref{alg:intersect:triangulation:hspace} further, for those polyhedrons that are marked as intersected by \cref{alg:dointersecterror} the truncated volume is computed. The polyhedron / halfspace intersection algorithm is outlined by \cref{alg:polyhedronhalfspace}. Intersection between the halfspace $H_c$ and each polygon $P$ of the polyhedron $V_c$ results in the intersectio polygon $P_{c,H_c}$ and intersection points $Y_{P_{c,H_c}}$ that are agglomerated into a global list of intersection points. This is necessary, because no order is imposed in the way multiset boundary representation of the polyhedron stores its polygons. Intersection points are then oriented using the \texttt{orient} algorithm and appended to the result multiset polyhedron $V_{c, H_c}$. This way, the last polygon in $V_{c,H_c}$ is always the cap polygon, the one that lies on the halfspace $H_c$, so that it can be accessed directy by \cref{alg:intersect:triangulation:hspace}. The \texttt{intersect\_error} algorithm is used for the polygon / halfspace intersection as well. It almost the same as \cref{alg:polyhedronhalfspace}: instead of polygons of the polyhedron, the algorithm loops over the edges of the polygons, intersects them, appends them to the result as well as the intersection points. The only difference is in adding the cap polygon: the multiset polygon resulting from polygon / halfspace intersection is implicitly closed. The \texttt{orient} algorithm used in \cref{alg:polyhedronhalfspace} is more complex. It orients the cap polygon in the negative direction of the halfspace normal, namely $-\n_c$. This is necessary, because the multiset representation of the polyhedron is an (unordered) set of polygons. Therefore, the intersection points resulting from the polygon / halfspace intersection are collected in no specific order. Furthermore, intersection points of the cap polygon that share edges and are duplicated by the multiset representation, will be very closely grouped and need to be welded together. 

\begin{algorithm}[htb]
    \centering
    \caption{Polyhedron / halfspace intersection}
    \label{alg:polyhedronhalfspace}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Polyhedron $V_c$, Halfspace $H_c$
            \State \textbf{Returns:} Volume of the intersection $|V_{c,H_c}|$, area of the cap polygon $A_{c,H_c}$ 
            \State Initialize the result polyhedron $V_{c, H_c}$
            \State Initialize the intersection points $X_{c}= \emptyset$
            \For {polygon $P$ in $V_c$}
                \State $(P_{c,H_c}, Y_{P_{c,H_c}}) = $ \texttt{intersect\_error}$(P, H_c)$  \Comment $Y_{P_{c,H_c}} :=$ set of intersection points of $P_{c,H_c}$.
                \If {$P_{c,H_c}$ is not \texttt{COPLANAR} with $H_c$}
                    \State $V_{c,H_c} = V_{c,H_c} \cup P_{c,H_c}$ \Comment Append intersection polygon to the result. 
                    \State $X_{c} = X_{c} \cup Y_{P_{c,H_c}}$ \Comment Append intersection points to $X_c$.
                \EndIf  
                \State $X^o_c = $ \texttt{orient}$(X_c)$ \Comment Orient intersection points to build the cap polygon.
                \State $V_{c,H_c} = V_{c,H_c} \cup X^o_c$ \Comment Append the cap polygon to the result. 
            \EndFor
            \State \Return $V_{c,H_c}$
      \end{algorithmic}
    }
\end{algorithm}

\begin{algorithm}[!htb]
    \centering
    \caption{Orient cap polygon points}
    \label{alg:orient}
    {\footnotesize
        \begin{algorithmic}[1]
            \State \textbf{Input:} Unordered points $X_c$ of the cap polygon, orientation normal $\n$
            \State \textbf{Returns:} Oriented cap polygon $X^o_c$ 
            \State Initialize $X^o_c = X_c$ 

            \State $\p_0 = $ first point $\in X^o_c$ 
            \State $\p_1 = $ second point $\in X^o_c$ 
            \State $\p_0\p_1 = \p_1 - \p_0$ 
            \State $s_{min} = MAX$ \Comment $MAX =$ largest positive double.
            \State $\p_{min} = (MAX, MAX,MAX)$ \Comment $\p_{min}=$ point $\r$ with max projection on $\p_0\p_1$. 
            \State $s_{max} = MIN$ \Comment $MIN =$ largest negative double.
            \State $\p_{max} = (MIN, MIN,MIN)$ \Comment $\p_{min}=$ point $\r$ with min projection on $\p_0\p_1$. 
            \For {every point $\r \in X^o_c$} \Comment Find minimal and maximal projections on $\p_0\p_1$.
                \State $s_r = (\r - \p_0) \cdot \p_0\p_1$ \Comment Projection of $\r$ onto $\p_0\p_1$.
                \If {$s_r < s_min$}
                    \State $\p_{min} = \r$
                    \State $s_{min} = s_r$
                \ElsIf {$s_r >= s_{max}$}
                    \State $\p_{max} = \r$ 
                    \State $s_{max} = s_r$
                \EndIf
            \EndFor
            \State $L^o_c = \emptyset$ \Comment Points left of $\p_0\p_1$.
            \State $R^o_c = \emptyset$ \Comment Points right of $\p_0\p_1$.
            \For {every point $\r \in X^o_c$} \Comment Categorize $X^o_c$ as above or below of $\p_{min}\p_{max}$. 
                \State $s_r = (\r - \p_0) \cdot \p_0\p_1$ \Comment Projection of $\r$ onto $\p_0\p_1$.
                \If {\texttt{left\_error}$(\p_{min}\r, \p_{min}\p_{max}, \n)$} \Comment $\r$ approximately left from $\p_{min}\p_{max}$.
                    \State $L^o_c = L^o_c \cup (\r, s_r)$
                \Else{}
                    \State $R^o_c = R^o_c \cup (\r, s_r)$
                \EndIf
            \EndFor
            \State $L^s_c = \texttt{sort\_ascending}(L^o_c)$ \Comment Sort by $s_r$ in ascending order.
            \State $L^w_c = \texttt{unique}(L^o_c)$ \Comment Weld together close points. 
            \State $R^s_c = \texttt{sort\_descending}(L^o_c)$ \Comment Sort by $s_r$ in descending order.
            \State $R^w_c = \texttt{unique}(R^o_c)$ \Comment Weld together close points. 
            \State $X^o_c = L^w_c \cup R^w_c$
            \State \Return $X^o_c$. 
      \end{algorithmic}
    }
\end{algorithm}

\Cref{alg:orient} outlines the core of the algorithm, handling the special case of a triangle or a quadrilateral is not shown. An alternative to \cref{alg:orient} would be an algorithm that computes the centroid of the polygon $\mathbf{c}_P$, and then uses $\mathbf{c}_P\p_0$ for $\p_0\p1$ and sorts the points clockwise while welding together close points. Profiling of the geometrical intersection using HPCToolkit \cite{Adhianto2010} has shown the orientation of the polygon is not the bottlenec, because \cref{alg:intersect:triangulation:hspace} intersects tetrahedra in the decomposition, which results in triangular or quadrilateral polygons that are easily handled by \cref{alg:orient} as special cases.

\Cref{alg:intersect:triangulation:hspace}, and its sub-algorithms used with the multiset models are straightforward to implement, because they do not require connectivity between vertices, edges or polygons of the geometrical models. Even \Cref{alg:orient}, although lengthy, is straightforward to implement, if the sorting and uniqueness operations are already available in a library of the used programming language (this is the case for C++ and STL). As mentioned already, the cost of of simplicity is the manipulation of additional duplicated data by the multiset model. The next section demonstrates the measured absolute computational costs incured by the multiset model when used with a novel iterative algorithm for the positioning of aVOF plane in a general star-shaped polyhedron that can be non-convex and have non-planar faces.  


==> sections/software_design.tex <==
\section{Software design}
\label{sec:software}

\texttt{Geophase} is a generic C++ library, that abstracts geometrical models and algorithms using C++ templates. The most basic idiom of generic programming with C++ templates is the so-called \emph{type lifting}, where the same algorithm template is used to instantiate code for different, most likely unrelated argument types. This is possible, if the operations that are performed by the algorithm are satisfied by the different types, and these operations therefore implicitly define the interface the types must satisfy. The implicit interface defines an abstract notion - a concept of a sort. A concept is not implemented in terms of the source code and is therefore fully abstract. An example of a concept would be a polygon sequence. In \texttt{geophase}, a polygon sequence is a sequence of polygons that provides access to each polygon using the STL iterator interface. An example model of the polygon sequence concept would be an STL-conform vector (or list, or double-ended queue) of polygon models. 

Types passed as template arguments to the type-lifted algorithm either satisfy the implicit interface prescribed by the algorithm template, or they do not. Those template arguments that satisfy the implicit interface can be used to instantiate a template, resulting in valid code. If an error occurs during the substitution of the template argument, the compiler \emph{does not produce an error and stop the compilation}, it continues to search through remainder of the set of available templates until such an template is found, which satisfies the implicit interface. This idiom of the C++ programming language is called Substitution Failure Is Not An Error (SFINAE) and the implementation \texttt{geophase} relies on it extensively. 

Relying solely on type lifting for the geometrical calculations is insufficient, because different geometrical algorithms may enforce the same implicit interface on different geometrical models. For example, computing the oriented area of a polygon using \cref{alg:area:oriented} can be done accidentally for a chain of line segments. If the list or the array model a chain of line segments instead of a polygon, the implicit interface defined in \cref{alg:area:oriented} remains the same, and an area of a chain of line segments is computed, which makes no sense. Therefore it becomes necessary to distinguish the chain of line segments from a closed polygon, even if they are using the same storage and provide the same access functions. If the algorithm requires the polygon type to only satisfy the STL sequence container interface, the compiler will find both the chain of line segments and the polygon to be equally valid. In the case where two such algorithms exist, an \emph{ambiguity error} occurs, as the compiler cannot decide between two equally viable function templates. 

\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            template <typename Polyhedron, typename RT = double>
            RT volume(Polyhedron const & p)
            {
                RT result(0); 

                auto C = center(p); 
                for (const auto& polygon : p) 
                    result += volume(C, p); 

                return result;
            }
\end{minted}
\caption{Volume calculation function template.} 
\label{lst:volume}
\end{listing}

A code example showing the ambiguity faced by the compiler when only type lifting is applied to the geometrical algorithm is shown in \cref{lst:volume}. Merely naming the template parameters differently does not make them different to the compiler. In the code shown in \cref{lst:volume}, the algorithm does not actually compute the volume of a polyhedron. The computation is valid \emph{for any model} that implements an STL iterator interface and for which the \texttt{volume(C, p)} algorithm is implemented. Defining multiple templates such as one in \cref{lst:volume} results in an ambiguity error.

In order to disambiguate algorithms, following approaches can be applied: \emph{tag dispatching} and \emph{concept-based function overloading}. 

\subsection{Tag dispatching}

Selection of algorithms can be enforced based on the specific properties of a template argument. Type properties, often called type traits, are implemented as concrete types as well, since the C++ template mechanisms are based on types. Multiple traits are bundled together in traits classes, that can then be used to select appropriate algorithms. Algorithms that are considered appropriate might be those optimized for efficiency for a specific model, or simply those that result with a valid code for the template argument (disambiguation). For example, the application of trait classes to selecting an optimal distance calculation between two iterators of the STL is described by \citet{Josuttis2012}, section $9.3.3$, page $445$. 

An example trait class is shown in \cref{lst:tag}, together with two concrete tag types: \path{polygon_collection_tag} and \path{polygon_sequence_tag}. 
%
\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            struct polygon_collection_tag {};  
            struct polygon_sequence_tag : polygon_collection_tag {};

            template<typename Geometry>
            struct tag; 

            template<>
            struct tag<PolygonSequence>
            {
                typedef polygon_sequence_tag type; 
            };
\end{minted}
\caption{Using type traits to tag geometrical models.} 
\label{lst:tag}
\end{listing}
%
Tag dispatching relies on a general function template, that obtains the tag of the template arguments from the tag trait class shown in \cref{lst:tag} and then dispatches the function call further on. The way the function call is dispatched is determined by the choice of the tag dispatching approach: value-based and type-based dispatching approaches. 

Value-based tag dispatching is shown in \cref{lst:valuetag} and relies on function overloading for tag types. Function overloading allows the tag dispatching system to introduce co-dependence between tags, such as inheritance which is shown in \cref{lst:tag}. For example, the polygon sequence is an ordered collection of polygons, and this relationship is modeled with the inheritance relationship between the respective tags. When value based dispatching is applied, as in the return statement in \cref{lst:valuetag}, that volume algorithm will be chosen among all candidates for which the tag objects are most specific. In other words: the derived tag types have precedence from the base tag types, as they are more specific. 

\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            template
            <
                typename GeometryOne, 
                typename GeometryTwo, 
                typename RT = double
            >
            RT volume(GeometryOne const & one, GeometryTwo const & two)
            {
                return volume(
                  one, 
                  tag<GeometryOne>::type(), 
                  two, 
                  tag<GeometryTwo>::type()
                );
            }
\end{minted}
\caption{Value based tag dispatch.}
\label{lst:valuetag}
\end{listing}

Type based tag dispatching uses tag types as template arguments for class (structure) templates and relies on the partial template specialization to provide alternative implementations. The type based tag dispatching approach is used by the \texttt{boost.geometry} library, and is covered in detail by \citet{bgboostcon2009} and \citet{bgboostcon2010}, as well as the official library documentation \citep{bgwiki165}. 

When type based tag dispatching is used, structure templates are implemented within a separate (dispatch) namespace, and calls to those algorithms are made by the generic dispatch function template similar to one in \cref{lst:valuetag}. \cref{lst:typetag} is an example of a type-based dispatch. 

\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            template
            <
                typename GeometryOne, 
                typename GeometryTwo, 
                typename RT = double
            >
            RT volume(GeometryOne const & one, GeometryTwo const & two)
            {
                return dispatch::volume
                <
                  typename tag<GeometryOne>::type, 
                  typename tag<GeometryTwo>::type
                >::apply(one, two);
            }
\end{minted}
\caption{Type based tag dispatch.}
\label{lst:typetag}
\end{listing}

Value tag dispatch (\cref{lst:valuetag}) and type tag dispatch (\cref{lst:typetag}) are similar to each other in the fact that they both rely on tags to disambiguate the algorithms that perform the calculations. The difference lies in the fact that the algorithms are implemented as static member functions for type based tag dispatching, and global functions for value based tag dispatching. Extending the algorithm set with a global function incurs less programming overhead than extending the dispatch namespace with a specialized structure template. Keeping the programming overhead low for structural enhancements of the implementation plays an important role both in maintenance and future extensions of the geometrical Volume-of-Fluid method. 

One issue with value based tag dispatching is that the number of function arguments grows with the introduction of tags. On the other hand, with type based tag dispatching, extending the set of available algorithms requires the user to implement a structure within the dispatch namespace. Both tag dispatching approaches also complicate the code for those algorithms that call on other algorithms. At each call site (e.g. polygon intersection called from within polyhedron intersection), a tag dispatch call must be implemented which results in surplus code that is used only to disambiguate algorithms.  

\subsection{Concept based function overloading}

The concept based overloading is not to be misinterpreted with C++ concepts as proposed by \citet{cppConceptProposal2011} and introduced as a part of the STL library with the C++20 standard. Instead, concept based overloading in the form of function overloading based on arbitrary properties of types as introduced by \citet{Jarvi2003} has been considered as a tool to disambiguate geometrical algorithms. The basic idea behind this mechanism is to use metafunctions to compute return types for the algorithms. In cases when the metafunction fails to compute the function return type, the SFINAE idiom forces the compiler to check the remainder of the function template set for a viable function template instantiation. 

\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            template
            <
                typename PointSequence, 
                typename Halfspace, 
                typename RT = double
            >
            typename return_type<Polygon, Halfspace>::RT 
            distance(Polygon const & poly, Halfspace const & hspace)
            {
                RT result; 

                // Operations on poly and hspace.

                return result; 
            }
\end{minted}
\caption{Polygon sequence / half-space distance.}
\label{lst:conceptoverload-pointseq}
\end{listing}

\begin{listing}
\centering
\begin{minted}[fontsize=\footnotesize]{c++}
            template
            <
                typename IndexedPolygon, 
                typename Halfspace, 
                typename RT = double
            >
            typename return_type<IndexedPolygon, Halfspace>::RT 
            distance(IndexedPolygon const & poly, Halfspace const & hspace)
            {
                RT result; 

                // Operations on poly and hspace.

                return result; 
            }
\end{minted}
\caption{Indexed polygon / half-space distance.}
\label{lst:conceptoverload-indexed}
\end{listing}

\Cref{lst:conceptoverload-indexed,lst:conceptoverload-pointseq} show two different template functions that implement the distance calculation between the polygon a half-space concepts. The example metafunction \path{return_type} returns either a specific return type based on properties of the parsed template arguments, or a void type. Since the functions return a result, a void type cannot be used and the template argument substitution fails to produce valid code. 

The metafunctions responsible for calculating the function template return type can be based on the implicit interface defined by the function implementation. This would be the most simple implementation of concepts in terms of metafunctions. However, in that case, the ambiguity is still not resolved in cases when multiple algorithms exist that prescribe the same implicit interfaces, as discussed for the \cref{lst:volume}. 

The way the metafunction \path{return_type} is implemented determines the behavior of the template instantiation process. \citet{Jarvi2003} have shown that the metafunctions can be combined with tags. In that case, no general function template is required that implements tag dispatching, as shown in \cref{lst:valuetag,lst:typetag} for value and type based tag dispatching, respectively. However, the benefit does not lie in removing a single generic function template for tag dispatching per set of algorithms. The main benefit lies in the dispatch call being completely removed from sub-algorithm call sites. This significantly increases code readability, reduces code bloat and improves software design scaling. 

Software design scaling\index{software design scaling} can be defined as a number of points in the source code that need to be modified (points of variation) \emph{additional} to the original source code extension driven by optimization, a new feature, etc. In cases when the new geometrical model can be efficiently used with existing algorithm function templates, there is one point of variation: tagging the model with the appropriate tag. When a new algorithm is to be added that works with existing concepts, there is one point of variation: implementing a function template enabled by the existing tags. In the case when both a new concept and a new algorithm are to be added, there are two points of variation: introducing a new tag, and programming a new function template. Therefore, the applied design to the geometrical Volume-of-Fluid method scales very well.  

Because of good design scaling, the design of the geometrical algorithms relies on using metafunctions in combination with tags as proposed by \citet{Jarvi2003}. Each concept involved in the geometrical calculation is therefore tagged with a tag. The main benefits of using function overloading based on argument properties combined with type tags for geometrical operations of the VOF method can be summarized as:

\begin{itemize}
  \item an algorithm implementation such as one partially shown in can be re-used with any STL-compliant container, 
  \item multiple algorithms are disambiguated easily (no additional namespace and no additional structure templates are required), 
  \item the design scales well (there is only one point of variation er algorithm and a new concept),
  \item different data structures and sub-algorithms can be interchanged without the overhead and complexity brought by dynamic polymorphism, 
  \item using templates enables the compiler to perform more effective efficiency optimizations, 
  \item new geometrical transport methods consisted of different sub-algorithms can be assembled simply by interchanging template arguments.
\end{itemize}

